Functional Failure Rate Due to Single-Event Transients in Clock Distribution Networks

With technology scaling, lower supply voltages, and higher operating frequencies clock distribution networks become more and more vulnerable to transients faults. These faults can cause circuit-wide effects and thus, significantly contribute to the functional failure rate of the circuit. This paper proposes a methodology to analyse how the functional behaviour is affected by Single-Event Transients in the clock distribution network. The approach is based on logic-level simulation and thus, only uses the register-transfer level description of a design. Therefore, a fault model is proposed which implements the main effects due to radiation-induced transients in the clock network. This fault model enables the computation of the functional failure rate caused by Single-Event Transients for each individual clock buffer, as well as the complete network. Further, it allows the identification of the most vulnerable flip-flops related to Single-Event Transients in the clock network. The proposed methodology is applied in a practical example and a fault injection campaign is performed. In order to evaluate the impact of Single-Event Transients in clock distribution networks, the obtained functional failure rate is compared to the error rate caused by Single-Event Upsets in the sequential logic.

==> pgflibraryshapes.gates.flipflops.IEC.code.tex <==





\usepgflibrary{shapes.gates.logic.IEC}

\pgfkeys{/pgf/.cd,
	flip flop is latch/.is if=pgfflipflopislatch,%
	flip flop bottom clock/.is if=pgfflipflopbottomclock,%
	flip flop D label/.initial=D,%
	flip flop Clk label/.initial=,%
	flip flop CE label/.initial=,%
	flip flop Q label/.initial=Q,%
	flip flop Qn visible/.is if=pgfflipflopqnvisible,%
	flip flop Qn label/.initial={$\overline{\mbox{Q}}$},%
	flip flop S label/.initial=,%
	flip flop R label/.initial=,%
	flip flop Clk inverted/.is if=pgfflipflopclkinverted,%
	flip flop CE inverted/.is if=pgfflipflopceinverted,%
	flip flop S inverted/.is if=pgfflipflopsinverted,%
	flip flop R inverted/.is if=pgfflipfloprinverted,%
}

\tikzset{flip flop/port labels/.style={font=\sffamily\small}}
\tikzset{every dff node/.style={%
	draw,%
	minimum width=1.5cm,%
	minimum height=2.0cm,%
	thick,%
	inner sep=1mm,%
	outer sep=0pt,%
	cap=round,%
	add font=\sffamily},%
}


\tikzset{add font/.code={%
	\expandafter\def\expandafter\tikz@textfont%
	\expandafter{\tikz@textfont#1}
	}
}

\newif\ifpgfflipflopislatch
\newif\ifpgfflipflopbottomclock
\newif\ifpgfflipflopqnvisible
\newif\ifpgfflipflopclkinverted
\newif\ifpgfflipflopceinverted
\newif\ifpgfflipflopsinverted
\newif\ifpgfflipfloprinverted

\pgfdeclareshape{dff}{
  \saveddimen\invertedradius{%
    \pgfmathsetlength{\pgf@x}{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
  }
  \saveddimen\outerinvertedradius{%
    \pgfmathsetlength{\pgf@x}{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	  \advance\pgf@x.5\pgflinewidth%
  }
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  \savedanchor\Clk{
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
    \pgf@x=-1\pgf@x%
    \ifpgfflipflopbottomclock%
      \pgf@y=-.5\pgf@y%
    \else%
      \pgf@y=0\pgf@y%
    \fi%
    \ifpgfflipflopclkinverted%
      \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
      \advance\pgf@xa.5\pgflinewidth%
      \advance\pgf@x-\pgf@xa%
      \advance\pgf@x-\pgf@xa%
    \else%
    \fi%
  }
  \savedanchor\CE{
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
    \pgf@x=-1\pgf@x%
    \ifpgfflipflopbottomclock%
      \pgf@y=0\pgf@y%
    \else%
      \pgf@y=-.5\pgf@y%
    \fi%
    \ifpgfflipflopceinverted%
      \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
      \advance\pgf@xa.5\pgflinewidth%
      \advance\pgf@x-\pgf@xa%
      \advance\pgf@x-\pgf@xa%
    \else%
    \fi%
  }
  \savedanchor\S{
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
    \pgf@x=0pt%
    \ifpgfflipflopsinverted%
      \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
      \advance\pgf@ya.5\pgflinewidth%
      \advance\pgf@y\pgf@ya%
      \advance\pgf@y\pgf@ya%
    \else%
    \fi%
  }
  \savedanchor\R{
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
    \pgf@x=0pt%
    \pgf@y=-\pgf@y%
    \ifpgfflipfloprinverted%
      \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
      \advance\pgf@ya.5\pgflinewidth%
      \advance\pgf@y-\pgf@ya%
      \advance\pgf@y-\pgf@ya%
    \else%
    \fi%
  }
  \savedanchor\Qn{
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
    \pgf@y=-.5\pgf@y%
    \ifpgfflipflopqnvisible%
      \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
      \advance\pgf@xa.5\pgflinewidth%
      \advance\pgf@x\pgf@xa%
      \advance\pgf@x\pgf@xa%
    \else%
    \fi%
  }
  \inheritanchorborder[from=rectangle]

  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{D}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.5\pgf@y%
  }
  \anchor{Clk}{\Clk}
  \anchor{CE}{\CE}
  \anchor{Q}{
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
  }
  \anchor{Qn}{\Qn}
  \anchor{S}{\S}
  \anchor{R}{\R}

  \backgroundpath{
    \pgfpathrectanglecorners{\southwest}{\northeast}
  }

  \foregroundpath{
    {
      \color{black}

      \pgfsetlinewidth{0.4pt}

      \pgf@anchor@dff@Clk
      \ifpgfflipflopclkinverted%
	\advance\pgf@x\outerinvertedradius%
	\advance\pgf@x\outerinvertedradius%
      \fi%
      \pgf@xa=\pgf@x \pgf@ya=\pgf@y
      \pgf@xb=\pgf@x \pgf@yb=\pgf@y
      \pgf@xc=\pgf@x \pgf@yc=\pgf@y
      \ifpgfflipflopislatch%
      \else%
	\tikzset{flip flop/port labels} %
	\tikz@textfont
	\pgfmathsetlength\pgf@x{1.6ex} %
	\advance\pgf@ya by .4\pgf@x
	\advance\pgf@xb by 1.1\pgf@x
	\advance\pgf@yc by -.4\pgf@x
	{
	  \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
	  \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
	  \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
	  %
	}
      \fi%

      \begingroup
      \tikzset{flip flop/port labels} %
      \tikz@textfont

      \pgf@anchor@dff@D
      \pgftext[left,base,at={\pgfpoint{\pgf@x}{\pgf@y}},x=\pgfshapeinnerxsep]{%
	\raisebox{-0.75ex}{\pgfkeysvalueof{/pgf/flip flop D label}}%
      }

      \pgf@anchor@dff@Clk
      \pgf@xc=\pgf@x
      \pgf@yc=\pgf@y
      \ifpgfflipflopclkinverted%
	\advance\pgf@xc\outerinvertedradius
	\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%
	\advance\pgf@xc\outerinvertedradius
      \fi
      \ifpgfflipflopislatch%
      \else
	\pgfmathsetlength\pgf@x{1.0ex} %
	\advance\pgf@xc\pgf@x
      \fi
      \pgftext[left,base,at={\pgfpoint{\pgf@xc}{\pgf@yc}},x=\pgfshapeinnerxsep]{%
	\raisebox{-0.75ex}{\pgfkeysvalueof{/pgf/flip flop Clk label}}%
      }

      \pgf@anchor@dff@CE
      \pgf@xc=\pgf@x
      \pgf@yc=\pgf@y
      \ifpgfflipflopceinverted%
	\advance\pgf@xc\outerinvertedradius
	\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%
	\advance\pgf@xc\outerinvertedradius
      \fi
      \pgftext[left,base,at={\pgfpoint{\pgf@xc}{\pgf@yc}},x=\pgfshapeinnerxsep]{%
	\raisebox{-0.75ex}{\pgfkeysvalueof{/pgf/flip flop CE label}}%
      }

      \pgf@anchor@dff@Q
      \pgftext[right,base,at={\pgfpoint{\pgf@x}{\pgf@y}},x=-\pgfshapeinnerxsep]{%
	\raisebox{-0.75ex}{\pgfkeysvalueof{/pgf/flip flop Q label}}%
      }

      \ifpgfflipflopqnvisible%
	\pgf@anchor@dff@Qn
	\pgf@xc=\pgf@x
	\pgf@yc=\pgf@y
	\advance\pgf@xc-\outerinvertedradius
	\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%
	\advance\pgf@xc-\outerinvertedradius
	\pgftext[right,base,at={\pgfpoint{\pgf@xc}{\pgf@yc}},x=-\pgfshapeinnerxsep]{%
	  \raisebox{-0.75ex}{\pgfkeysvalueof{/pgf/flip flop Qn label}}%
	}
      \fi

      \pgf@anchor@dff@S
      \pgf@xc=\pgf@x
      \pgf@yc=\pgf@y
      \ifpgfflipflopsinverted%
	\advance\pgf@yc-\outerinvertedradius
	\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%
	\advance\pgf@yc-\outerinvertedradius
      \fi
      \pgftext[top,at={\pgfpoint{\pgf@xc}{\pgf@yc}},y=-\pgfshapeinnerysep]{%
	\pgfkeysvalueof{/pgf/flip flop S label}%
      }

      \pgf@anchor@dff@R
      \pgf@yx=\pgf@x
      \pgf@yc=\pgf@y
      \ifpgfflipfloprinverted%
	\advance\pgf@yc\outerinvertedradius
	\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%
	\advance\pgf@yc\outerinvertedradius
      \fi
      \pgftext[bottom,at={\pgfpoint{\pgf@xc}{\pgf@yc}},y=\pgfshapeinnerysep]{%
	\pgfkeysvalueof{/pgf/flip flop R label}%
      }
      \endgroup
      \pgfusepath{stroke}
    }
  }

}


\endinput

